LiDARNet: A Boundary-Aware Domain Adaptation Model for Point Cloud Semantic Segmentation

We present a boundary-aware domain adaptation model for LiDAR scan full-scene semantic segmentation (LiDARNet). Our model can extract both the domain private features and the domain shared features with a two-branch structure. We embedded Gated-SCNN into the segmentor component of LiDARNet to learn boundary information while learning to predict full-scene semantic segmentation labels. Moreover, we further reduce the domain gap by inducing the model to learn a mapping between two domains using the domain shared and private features. Additionally, we introduce a new dataset (SemanticUSL\footnote{The access address of SemanticUSL:\url{https://unmannedlab.github.io/research/SemanticUSL}}) for domain adaptation for LiDAR point cloud semantic segmentation. The dataset has the same data format and ontology as SemanticKITTI. We conducted experiments on real-world datasets SemanticKITTI, SemanticPOSS, and SemanticUSL, which have differences in channel distributions, reflectivity distributions, diversity of scenes, and sensors setup. Using our approach, we can get a single projection-based LiDAR full-scene semantic segmentation model working on both domains. Our model can keep almost the same performance on the source domain after adaptation and get an 8\%-22\% mIoU performance increase in the target domain.

==> algorithms/algorithm1.tex <==
\begin{algorithm}[H]
    \caption{Range Image Preprocessing }
    \label{alg:algorithm1}
    \begin{algorithmic}
      \INPUT$I_{\text{mask}}$, $I_{\text{range}}$, $I_{\text{label}}$,$I_{\text{reflectivity}}$}.
      \STATE{$\hat{I}_{\text{mask}} = Closing(I_{\text{mask}})$}
      \STATE{$I_{\text{stripe}} = \hat{I}_{\text{mask}} - I_{\text{mask}}$}
      \STATE{$\hat{I}_{\text{range}} = NSInpainting(I_{\text{range}},I_{\text{stripe}})$}
      \STATE{$\hat{I}_{\text{reflectivity}} = NSInpainting(I_{\text{reflectivity}},I_{\text{stripe}})$}
      \STATE{$\hat{I}_{\text{label}} = NNInpainting(I_{\text{label}},I_{\text{stripe}})$}
    \end{algorithmic}
  \end{algorithm}

==> equations/conversion_st.tex <==
\begin{equation}
    \label{eqn:conversion_st}
    G_{S \to T}(X)=f_{S \to T}(f_D(f_H(x_s),f_C(f_H(X)))
\end{equation}

==> equations/conversion_ts.tex <==
\begin{equation}
    \label{eqn:conversion_ts}
    G_{T \to S}(X)=f_{T \to S}(f_D(f_H(x_t),f_C(f_H(X)))
\end{equation}

==> equations/cyc_outputs.tex <==
\begin{equation}
  \begin{split}
    \hat{x}_{s(t)} & = G_{T \to S}(x_t) \\
    & =f_{T \to S}(f_D(f_H(x_t),f_C(f_H(x_t)))
  \end{split}
\end{equation}
\begin{equation}
  \begin{split}
    \hat{x}_{t(s)} & = G_{S \to T}(x_s) \\
    & =f_{S \to T}(f_D(f_H(x_s),f_C(f_H(x_s)))
  \end{split}
\end{equation}
\begin{equation}
  \begin{split}
    \hat{x}_{s(s)} & = G_{T \to S}(x_s) \\
    & =f_{T \to S}(f_D(f_H(x_s),f_C(f_H(x_s)))
  \end{split}
\end{equation}
\begin{equation}
  \begin{split}
    \hat{x}_{t(t)} & = G_{S \to T}(x_t) \\
    & =f_{S \to T}(f_D(f_H(x_t),f_C(f_H(x_t)))
  \end{split}
\end{equation}
\begin{equation}
  \begin{split}
    \hat{x}_{t(s(t))} & = G_{S \to T}(\hat{x}_{s(t)}) \\
    & =f_{S \to T}(f_D(f_H(\hat{x}_{s(t)}),f_C(f_H(\hat{x}_{s(t)})))
  \end{split}
\end{equation}
\begin{equation}
  \begin{split}
    \hat{x}_{s(t(s))} & = G_{S \to T}(\hat{x}_{t(s)}) \\
    & =f_{S \to T}(f_D(f_H(\hat{x}_{t(s)}),f_C(f_H(\hat{x}_{t(s)})))
  \end{split}
\end{equation}

==> equations/definition.tex <==
Definition:
Input: source data \(X_S\), target data \(X_T\) \\

Ground Truth: \(Y_S\) \(B_S\) \\

Output: \(\hat{Y}_S\) \(\hat{Y}_T\) \(\hat{Y}_{S(T)}\) \(\hat{Y}_{T(S)}\) \\
        \(\hat{B}_S\) \(\hat{B}_T\) \(\hat{B}_{S(T)}\) \(\hat{B}_{T(S)}\) \\
        \(\hat{X}_{S(T)}\) \(\hat{X}_{T(S)}\) \(\hat{X}_{S(S)}\) \(\hat{X}_{T(T)}\)

Generator: \\
Boundary Generator: \(G_B(X) = f_C(f_H(X))\) \\
Label Generator: \(G_L(X) = f_{Seg}(f_C(f_H(X)))\) \\
Mapping \(S\to T\): \(G_{S\to T} = f_{S\to T}(f_C{f_H(X)},f_D{f_H(X)})\) \\
Mapping \(T\to S\) \(G_{T\to S} = f_{T\to S}(f_C{f_H(X)},f_D{f_H(X)})\)\\
Discriminator:\\
Label Discriminator: \(D_L\) \\
Source Discriminator:\(D_S\) \\
Target Discriminator: \(D_T\) \\
Boundary Discriminator: \(D_B\) \\

Boundary GAN Loss: \\
\(L_{GAN}(G_B,D_B,B_S,\hat{B}_T)\) \\

Label GAN Loss: \\
\(L_{GAN}(G_L,D_L,Y_S,\hat{Y}_T)\) \\

mapping \(G: S \to T\):\\
\(L_{GAN}(G_{S\to T},D_S,X_S,\hat{X}_{S(T)})\) \\

GAN mapping \(G: T \to S\):\\
\(L_{GAN}(G_{T\to S},D_T,X_T,\hat{X}_{T(S)})\) \\

==> equations/seg_s_loss.tex <==
\begin{equation}
    \label{eqn:seg_s_loss}
        L_{Seg}^{S}   = \lambda_{SS1}L_{CE}(Y_S,\hat{Y}_S) + \lambda_{SS2}L_{dual}(Y_S,\hat{Y}_S,\hat{B}_S) 
\end{equation}

==> figures/cyc_res.tex <==
\begin{figure*}[h]
    \vspace{0.1cm}
    \centering
    \includegraphics[width=0.9\textwidth]{./images/cyc_res.png}
    \caption{Input Representation and Corresponding Results: (a) are the range images; (b) are the reflectivity images; (c) are the co-ordinate maps; (d) are the normal maps; (e) are the predicted labels; (d) are the predicted boundaries. Columns 1 and 3 are the original target and source data; Columans 2 and 4 are the conversion results of cyc mechanism. }
    \label{fig:cyc_res}
\end{figure*}

==> figures/inpaint.tex <==
\begin{figure*}[h]
    \includegraphics[width=\textwidth]{inpaint.png}
    \caption{Inpainting Process. (a) the mask image;  (b) the closed mask; (c) the stripe position; (d) the original reflectivity image; (e) the original label; (f) the inpainted reflectivity image; (g) the inpainted label }
    \label{fig:inpaint}
\end{figure*}

==> figures/inpaint2.tex <==
\begin{figure}[h]
    \includegraphics[width=0.5\textwidth]{inpaint2.png}
    \caption{Inpainting Process. (a) the mask image;  (b) the closed mask; (c) the stripe position; (d) the original reflectivity image; (e) the original label; (f) the inpainted reflectivity image; (g) the inpainted label }
    \label{fig:inpaint}
\end{figure}

==> figures/inpaint3.tex <==
\begin{figure}[h]
    \includegraphics[width=0.5\textwidth]{inpaint3.png}
    \caption{Inpainting Process. (a) the original label; b) the inpainted label; (c) the original reflectivity image; (d) the inpainted reflectivity image; }
    \label{fig:inpaint}
\end{figure}

==> figures/input_represenation.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{input_representation}
  \caption{Projected Lidar Point Cloud Representation: (a) is range image; (b) is normal map; (c) is reflectivity image; (d)~(f) is co-ordinate image}
  \label{fig:input_representation}
\end{figure}

==> figures/network_structure.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{./images/network_structure.jpg}
    \caption{Network Structure}
    \label{fig:network_structure}
\end{figure*}

==> figures/point_cloud_campus.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
    \centering
    \includegraphics[width=0.95\textwidth]{point_cloud_campus}
    \captionof{figure}{(a) is ground truth point cloud of Texas A\&M Univerisity; (b) is point cloud point cloud of Texas A\&M Univerisity}
\end{center}%
}]

==> figures/point_cloud_campus_b.tex <==
\begin{figure*}[b]
    \includegraphics[width=0.95\textwidth]{point_cloud_campus}
    \caption{(a) is ground truth point cloud of Texas A\&M Univerisity; (b) is point cloud point cloud of Texas A\&M Univerisity}
    \label{fig:point_cloud_campus}
  \end{figure*}

==> figures/point_cloud_offroad.tex <==
\begin{figure*}[h]
  \includegraphics[width=0.95\textwidth]{point_cloud_offroad}
  \caption{Point Cloud Segmentation Results. (a) is the ground truth point cloud in off-road environment; (b) is predicted point cloud in off-road enviroment}
  \label{fig:point_cloud_results}
\end{figure*}

==> figures/point_cloud_results.tex <==
\begin{figure*}[h]
  \vspace{0.1cm}
  \centering
  \includegraphics[width=0.95\textwidth]{point_cloud_results}
  \caption{Point Cloud Segmentation Results. (a) is the ground truth point cloud in off-road environment; (b) is the predicted point cloud in off-road enviroment; (c) is the ground truth point cloud of Texas A\&M Univerisity; (d) is the predicted point cloud of Texas A\&M Univerisity}
  \label{fig:point_cloud_results}
\end{figure*}

==> figures/seg_res.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{seg_res.png}
    \caption{Segmentation results. (a) is the reflectivity image;  (b) is the baseline results; (c) is the baseline+normal results; (d) is the adaptation results; (e) is the adaptation+normal results; (f) is the ground truth}
    \label{fig:seg_res}
\end{figure*}

==> figures/warthog.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{warthog2}
  \caption{Our platform for collecting data}
  \label{fig:warthog}
\end{figure}
